On the Impact of Communities on Semi-supervised Classification Using Graph Neural Networks

Graph Neural Networks (GNNs) are effective in many applications. Still, there is a limited understanding of the effect of common graph structures on the learning process of GNNs. In this work, we systematically study the impact of community structure on the performance of GNNs in semi-supervised node classification on graphs. Following an ablation study on six datasets, we measure the performance of GNNs on the original graphs, and the change in performance in the presence and the absence of community structure. Our results suggest that communities typically have a major impact on the learning process and classification performance. For example, in cases where the majority of nodes from one community share a single classification label, breaking up community structure results in a significant performance drop. On the other hand, for cases where labels show low correlation with communities, we find that the graph structure is rather irrelevant to the learning process, and a feature-only baseline becomes hard to beat. With our work, we provide deeper insights in the abilities and limitations of GNNs, including a set of general guidelines for model selection based on the graph structure.

==> ablation.tex <==

%\section{Experimental study}
\subsection{Ablation study}
\label{sec:ablation}
After establishing the intuitions behind the role of communities, we aim to show their impact experimentally.
To achieve this, we evaluate five popular state-of-the-art GNN models on six empirical datasets. Subsequently, we re-evaluate these GNN models on the same datasets after applying ablation to their structures.

In particular, we evaluate the accuracy of GNNs on the original datasets and compare this performance to the ones on the following ablation models:
%, summarized in Table~\ref{tab:ablation-models}\hussain{is the table even necessary}:
\begin{itemize}
    \item \textbf{SBM networks.} Here we aim to rebuild the graph while preserving the communities. Thus, we firstly perform community detection with widely used Louvain method~\cite{louvain}, which maximizes the modularity score. Secondly, we build a stochastic block matrix encoding the original density of edges within and between the detected communities. Finally, we use this matrix to construct a graph with the stochastic block model (SBM)~\cite{holland1983stochastic}. This graph preserves a node's community, features and label but results in a binomial degree distribution~\cite{karrer2011stochastic}.%, effectively reducing the skew in the degree distribution.
    \item \textbf{CM networks.} In this ablation model, we apply graph rewiring using the so called configuration model (CM)~\cite{confmodel}.
    With this rewiring, each node keeps its degree, but its neighbors can become any of the nodes in the graph.
    This effectively destroys the community structure, while keeping the node's degree, features and label.
    \item \textbf{Random networks.} We use Erd{\H{o}}s-R{\'e}nyi graphs~\cite{erdos1960evolution} to eliminate both communities and degree distribution.
    The resulting graph has no community structure and features a binomial degree distribution.
This ablation model can only spread noisy feature information across the graph.
\end{itemize}

%\subsection{Uncertainty coefficient}
%As we have suggested using the uncertainty coefficient to quantify the cluster assumption, we compute our proposed measure for each of the studied datasets.
Last but not least, for each of the original datasets and each of the ablation models we compute the community-label correlation by means of the uncertainty coefficient.
To that end, we use the joint distribution of labels $L$ and communities $C$ (extracted by the Louvain method) to compute this coefficient for each graph.
In order to highlight the correlation between this coefficient and the applicability of GNNs, we show the computed coefficients on the given datasets along with their performance.


% (a) eliminating the skew in the degree distribution while preserving communities, (b) eliminating community structure while preserving the degree distribution, and (c) eliminating both structures by generating a graph completely at random.
% We compare the accuracy of the considered GNNs on each of these ablation models to their accuracy without ablation, i.e., on the original graphs.
% This leaves us with four choices of manipulation for each of the given graphs.

% \begin{table} [b]
% \label{tab:ablation-models}
% \centering
% \caption{Summary of ablation strategies. Random graphs only preserve the number of nodes and maintain an approximate edge density as in the original graph.}
% \begin{tabular}{cccl}
%     \toprule
%      \thead{Ablation\\model} & \thead{Community\\structure} & \thead{Degree\\distribution} & \thead{Ablation\\strategy}\\
%      \midrule
%      Original & \cmark & \cmark & \multicolumn{1}{c}{---} \\
%      SBM & \cmark & \xmark & Preserve communities \\
%      CM & \xmark & \cmark & Preserve hubs\\
%      Random & \xmark & \xmark & No preservation\\
%      \bottomrule
% \end{tabular}

% \end{table}

% \para{Original graphs.}
% With this choice, we apply no manipulation to the given graph.
% This represents the typical performance of GNNs on the given datasets and acts as a regulator to the following ablation models.

% \para{Preserving communities.}
% % graph communities seem to intuitively correlate with labels in some of our graphs: namely, the citation graphs,  (refer to Section~\ref{sec:information-theory} for a deeper view).
% In this ablation model, we aim to preserve community structure while reducing the length of the tail, \textit{and thus reducing the skew in the degree distribution implying the removal of hubs}~\cite{barabasi2013network} \hussain{perhaps find another reason/effect?}.
% To achieve this, we firstly perform community detection with widely used Louvain method~\cite{louvain}. This method maximizes the modularity score for each community. Modularity score measures the density of edges inside communities compared to edges between communities.
% Secondly, we build a stochastic block matrix encoding the density of edges within and between the detected communities
% (see Appendix~\ref{app:sbm-ablation} for details).
% Finally, we use this stochastic matrix to construct a graph with the stochastic block model (SBM)~\cite{holland1983stochastic}.
% This graph preserves a node's \textbf{community} as well as its features and label and results in a Poisson degree distribution~\cite{karrer2011stochastic}, effectively reducing the skew in the degree distribution.
% %\dhe{the degree distribution of sbms is not uniform but it is a mixture of binomials. try finding a reference for this. one of the mark newman papers should mention this for sure.} \hussain{in the worked I've cited (https://arxiv.org/pdf/1008.3926.pdf) they mention that the non-corrected model, which apparently is used by networkx, results in a Poisson degree distribution. I think it's fine to leave it this way, or do you think we should mention that the new degree distibution is poisson?}
% We refer to the graphs of this ablation model as the \textbf{SBM graphs}.

% \para{Preserving hubs.\hussain{degree dist.?}}
% In this ablation model, we apply graph rewiring using the so called configuration model (CM)~\cite{confmodel}.
% With this rewiring, each node keeps its degree, but its neighbors can become any of the nodes in the graph.
% As a result of keeping node degrees, hubs are preserved, and with rewiring, we eliminate community structure.
% We refer to these graphs as the \textbf{CM graphs}.

% \para{Completely random graphs.}
% Aiming for a full ablation, we construct $d$-regular random graphs~\cite{steger1999generating} to eliminate both communities and degree distribution.
% The constructed graphs are regular graphs with no self-loops or double edges.
% Using the method in~\cite{steger1999generating}, we generate random $d$-regular graphs, where all nodes have approximately degree $d$ up to a small statistical fluctuation \textit{(i.e, no hubs)}, and no particular community structure is realized.
% % \dhe{you can just state here that we use a standard Bernoulli random graph, which has a binomial degree distribution and no community structure. As a reference look for the original paper by Erdos und Renyi from late 50s.}\hussain{I couldn't verify that random $d$-regular graphs also follow binomial degree distribution, I think the nodes should have more or less a constant degree in that case, but I guess this anyway means having no particular community structure or hubs. If this is not enough, I can quickly build graphs with Erdos-Renyi method and report them instead} \dhe{sorry, i misunderstood this in the first iteration. you use d-regular random graphs and they aim at all nodes having degree d $\pm$ some statistical fluctuation. we can leave it at d-regular random graphs and you can just delete all the comments on this.}
% The only properties kept in these generated graphs are the set of nodes with their feature vectors and the approximate edge density.
% The intuition of such a construction is that it can only spread noisy feature information across the graph.
% Therefore, we look at this ablation model as a baseline for other ablation models.
% In this work, we will simply refer to graphs generated by this algorithm as \textbf{random graphs}.

\subsection{Experiments}
%\para{Evaluated models.}
In our experiments~\footnote{The implementation and technical details can be found on \url{https://github.com/sqrhussain/structure-in-gnn}}, we study five GNN architectures which are widely used for semi-supervised classification on graphs:
\begin{enumerate*}[label=(\alph*)]
    \item Graph Convolutional Networks (GCN)~\cite{gcn},
    \item Graph Sample and Aggregate (SAGE)~\cite{graphsage},
    \item Graph Attention Networks (GAT)~\cite{gat},
    \item Simple Graph Convolutions (SGC)~\cite{sgc}, and
    \item Approximate Personalized Propagation of Neural Predictions (APPNP)~\cite{Klicpera2019predict}%\footnote{Details about these works can be found in the respective papers.}.
\end{enumerate*}.
We additionally compare these approaches to a simple feature-only baseline, i.e., logistic regression model, which ignores the graph structure and only uses the node features.
The comparison to this baseline can indicate whether a GNN model is actually useful for the task on the respective datasets.


\para{Datasets.}
\label{sec:datasets}
To provide a better understanding of the roles of the studied structures, we aim for a diverse selection of datasets with respect to
\begin{enumerate*}[label=(\alph*)]
    \item domain, e.g., citation, social and web graphs,
    \item structure, e.g., directed acyclic vs. cyclic,
    \item and correlations between communities and labels, i.e., whether nodes of the same community tend to share the same label. 
\end{enumerate*}
Having this in mind, we use the datasets summarized in Table~\ref{tab:datasets}.

\begin{table}[b!]
\scriptsize
\caption{Dataset statistics after preprocessing (similar to Shchur et al.~\cite{shchur2018pitfalls}). The label rate represents the fraction of nodes in the \textit{training} set. The edge density is the number of existing undirected edges divided by the maximum possible number of undirected edges (ignoring self-loops). For Twitter dataset, we apply cleaning to the feature vectors of nodes same as in~\cite{Tiao2019}, i.e., removing graph-based and some textual features. }
\label{tab:datasets}
\centering
\begin{tabular}{lrrrrrr}
\toprule
Dataset & Labels & Features & Nodes & Edges & Edge density & Label rate \\
\midrule
CORA-ML~\cite{sen2008collective} & 7 & 1,433 & 2,485 & 5,209 & 0.0017 & 0.0563 \\
CiteSeer~\cite{sen2008collective} & 6 & 3,703 & 2,110 & 3,705 & 0.0017 & 0.0569 \\
PubMed~\cite{pubmed} & 3 & 500 & 19,717 & 44,335 & 0.0002 & 0.0030 \\
CORA-Full~\cite{corafull} & 67 & 8,710 & 18,703 & 64,259 & 0.0004 & 0.0716 \\
Twitter~\cite{twitter} & 2 & 215 & 2,134 & 7,040 & 0.0031 & 0.0187 \\
WebKB~\cite{webkb} & 5 & 1,703 & 859 & 1,516 & 0.0041 & 0.0582 \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[b]
% \label{tab:datasets}
% \centering
% \begin{tabular}{lrrrrrr}

% \toprule
% Dataset & Labels & Features & Nodes & Edges & Edge density & Label rate \\
% \midrule
% CORA-ML~\cite{sen2008collective} & 7 (topic) & 1,433 & 2,485 (papers) & 5,209 & 0.0017 & 0.0563 \\
% CiteSeer~\cite{sen2008collective} & 6 (topic) & 3,703 & 2,110 (papers) & 3,705 & 0.0017 & 0.0569 \\
% PubMed~\cite{pubmed} & 3 (topic) & 500 & 19,717 (papers) & 44,335 & 0.0002 & 0.0030 \\
% CORA-Full~\cite{corafull} & 67 (topic) & 8,710 & 18,703 (papers) & 64,259 & 0.0004 & 0.0716 \\
% Twitter~\cite{twitter} & 2 (hatefulness) & 215 & 2,134 (users) & 7,040 & 0.0031 & 0.0187 \\
% WebKB~\cite{webkb} & 5 (page type) & 1,703 & 859 (web pages) & 1,516 & 0.0041 & 0.0582 \\
% \bottomrule
% \end{tabular}
% \end{table}


%\para{Datasets description.}
%\label{sec:dataset-interest}
The label of a node in a \textit{citation graph} (i.e., \textit{CORA-ML, CiteSeer, PubMed} and \textit{CORA-Full}) represents the topic of the paper. Citations are expected to be denser among papers with similar topics than they would be between papers of different topics. For example, a publication about natural language processing would be more likely to cite other natural language processing papers than human-computer interaction papers. Therefore, one could intuitively expect that papers within the same graph community tend to share the same label.

\textit{Twitter} graph consists of users where the edges represent retweets, and node labels indicate whether a user is hateful or not.
Therefore, one could not easily assume the presence or the absence of a correlation between communities and labels (hateful or normal). In other words, we do not know whether hateful users typically form communities as this highly depends on the discussion topics.

For \textit{WebKB} dataset, nodes are web pages, edges are links, and labels indicate the type of the web page, i.e., course, faculty, project, staff or student.
In this case one cannot intuitively assume that nodes within a graph community are expected to share a label.
For example, a web page of a staff member could be more likely to link to projects on which this staff member is working than to other staff members' web pages.
Based on these intuitions, we consider that these graphs are sufficiently diverse concerning community impact on label prediction.% (more support to our assumption in Section~\ref{sec:uncertainty-result}).



\para{Evaluation setup}.
While the original graphs are directed, we treat them as undirected by ignoring the edge direction (which is in the line with previous research~\cite{graphsage,gcn,shchur2018pitfalls}).
All of these graphs are preprocessed in a similar manner as Shchur et al.~\cite{shchur2018pitfalls}, i.e., removing nodes with rare labels and selecting the largest weakly connected component except in WebKB where we take four connected components representing 4 universities.
Following the train/validation/test split strategy as in~\cite{shchur2018pitfalls}, each random split consists of $50$ labeled examples per class ($20$ for training and $30$ for validation) and the rest are considered test examples.
This applies to all of our datasets except WebKB where we use $10$ training examples and $15$ validation examples per class due to the fewer number of nodes.
To evaluate the GNN models on the original graphs, we follow the evaluation setup as conducted in~\cite{shchur2018pitfalls} by having $100$ random splits and $20$ random model initializations for each split.
The same process is carried out to evaluate the feature-only baseline (logistic regression) model.
The evaluation is slightly different for the ablation studies (SBM, CM and random graphs) since they include an additional level of randomization.
For a given dataset, we generate SBM, CM and random graphs with $10$ different random seeds, which results in $10$ SBM graphs, $10$ CM graphs and $10$ random graphs.
The evaluation on each of these generated graphs is carried out through $50$ different random splits and $10$ different random initializations.
As a result, the reported accuracy for a GNN architecture on the original graph is presented for $2,000$ trainings of the GNN.
Meanwhile, the reported accuracy of a GNN architecture on one of the ablation models (SBM, CM or random graphs) is presented for training the GNN $5,000$ times, i.e., $10$ randomly generated graphs $\times$ $50$ random splits $\times$ $10$ random initializations.

\para{Uncertainty coefficient calculation.}
To calculate $U(L|C)$ for a set of nodes, the labels of these nodes must be available.
% In a real-life scenario, the only known labels are the labels of nodes in the training and the validation set, while the labels of nodes in the test set are unknown.
Therefore, for each dataset, we compute $U(L|C)$ using the labeled nodes from the training and validation sets.%\dhe{i deleted all the comments and the second part of this description. i would now simply write the uncertainty coefficient everywhere and remove this distinction between empirical and estimated. this means you want to remove $\hat{U}$ and use simply $U$ everywhere. don't forget to update the figure 2 as well and remove the blue line in the upper row} 
%We denote this measure as $\hat{U}(L|C)$, and we later show that it correlates with the original one on the empirical datasets at hand. We report the mean value of $\hat{U}(L|C)$ on the different splits for each dataset. \dhe{this is not clear completely. do you mean .... using only the labeled nodes from the train and validation set?}\hussain{Is the explanation clear now? the labeled nodes are the nodes in the training and the validation set, when a node is unlabeled this means it's in the test set} \dhe{another question: does not this apply also for the calculation of the uncertainty coefficient in the original graph and in the ablation models as well? why do we compute the uncertainty coefficient in this way only for the perturbation of the SBM graphs? If we use two different computations: it maybe be better to decide on one computation and use it in all experiments. this we can discuss tomorrow} \hussain{I now use the estimated measure for all cases, please check}
%This estimate $\hat{U}(\hat{L}|\hat{C})$ will be computed similarly, but with $\hat{L}$ and $\hat{C}$ being the labels and communities of those labeled nodes instead of all nodes.
%Since the labeled nodes are sampled uniformly from each label, we assume that this estimated metric correlates with the actual one.
%So we use this estimated value and study its correlation with the GNN accuracy as we increase the community perturbations.




==> background.tex <==
\section{Background}
% \hussain{what should be in this section?}
\para{Graph neural networks.}
Let $G=(V,E)$ be a graph with a set of nodes $V$ and a set of edges $E$.
Let each node $u \in V$ have a feature vector $x_u \in \RR^d$, where $d$ is the feature vector dimension; and a label $y_u \in \mathcal{L}$, where $\mathcal{L}$ is the set of labels.
%\para{Graph neural networks.}

GNNs are multi-layer machine learning models, which operate on graphs.
They follow a message passing and aggregation scheme where nodes aggregate the messages that are received from their neighbors and update their representation on this basis.
In a GNN with $K$ hidden layers (with the input layer denoted as layer $0$), each node $u$ has a vector representation $h_u^{(k)}$ at a certain layer $k \leq K$ of dimension $d_k$.
The transformation from a layer $k$ to the next layer $k+1$ is performed by updating the representation of each node $u$ as follows:
\begin{equation}
    \label{eq:gnn}
    \begin{split}
    a_u^{(k)} & := \text{AGGREGATE}_{v \in \mathcal{N}(u)}(h_v^{(k)}),\\
    h_u^{(k+1)} & := \text{COMBINE}(h_u^{(k)},a_u^{(k)}),
    \end{split}
\end{equation}
where $\mathcal{N}(u)$ is the set of neighbors of $u$.
The AGGREGATE function takes an unordered set of vectors of dimension $d_k$ as an input, and returns a single vector of the same dimension $d_k$, e.g., element-wise mean or max.
The COMBINE function combines the representation of $u$ in layer $k$ with the aggregated representation of its neighbors, e.g.,  a concatenation followed by ReLU of a linear transformation $\text{COMBINE}(h,a) = \text{ReLU}(W.[h,a])$.
We set the representation of $u$ in the input layer to the input features: $h_u^{(0)} := x_u$.
In classification problems, the dimension of the last layer $d_K$ equals the number of labels in the graph $|\mathcal{L}|$.

\para{Semi-supervised learning on graphs.}
Semi-supervised learning aims to exploit unlabeled data in order to generate predictions given few labeled data.
In graphs, this means exploiting the unlabeled nodes as well as the network structure to improve the predictions.
Many semi-supervised classification methods on graphs assume that connected nodes are more likely to share their label~\cite{Li2018Deeper}, which is usually referred to as the \textit{cluster assumption}~\cite{chapelle2009semi}.  
Based on this assumption, approaches to solve this task usually aim to propagate node information along the edges.
Earlier related approaches~\cite{sen2008collective,zhu2003semi} focused on propagating label information from labeled nodes to their neighbors.
In many applications, however, graph nodes can also be associated with feature vectors, which can be utilized by GNNs.
GNNs achieved a significant improvement over the state of the art since they can effectively harness the unlabeled data, i.e., graph structure and node features.
%Next we will analyze the cluster assumption and how it relates to the way how GNNs solve classification task om graphs.

%\section{Cluster Assumption}
% \para{Semi-supervised classification with GNNs.} \hussain{not sure whether to put this subsection in the bg section}
% Semi-supervised classification on graph data aims to exploit the graph structure in order to perform predictions given a few labeled nodes.
% \para{Feature smoothing.}
\para{Cluster assumption.} GNNs operate by propagating node feature vectors along the edges, hence exploiting both the graph structure and feature vectors. %, enabling them to improve the state of the art on the semi-supervised classification task.
The GNN update rule in Equation~\ref{eq:gnn} can be seen as a form of \textit{(Laplacian) feature smoothing}~\cite{Li2018Deeper} as it combines the feature vector of a node with the feature vectors of its neighbors.
Feature smoothing results in neighboring nodes having similar vector representations.
Therefore, with the cluster assumption in mind, feature smoothing potentially causes nodes with similar labels to also obtain similar vector representations.
However, when the cluster assumption does not hold, i.e., connected nodes are less likely to share their label, the propagation in Equation~\ref{eq:gnn} can cause nodes with different labels to have similar vector representations.
It is widely accepted that classifiers achieve better accuracy when similar vector representations tend to have similar labels.
% Therefore, propagation while the cluster assumption holds could ease the classification task, while it could hinder it when the cluster assumption is not valid.

\para{Communities and the cluster assumption.}
Communities are densely connected subgraphs, and they are common in empirical graphs including social, citation or web graphs.
The existence of communities directly affects information propagation in graphs~\cite{cherifi2019community}.
As communities are densely connected, the feature smoothing performed by the update rule in Equation~\ref{eq:gnn} tends to make nodes within the same community have similar vector representations.
This dense connectivity also causes the cluster assumption to generalize to the community level, which means that nodes within the same community tend to share the same label.
As a result, when the cluster assumption holds, GNNs cause nodes with the same label to have similar vector representations simplifying the classification task on the resulting vector representations. Li et al.~\cite{Li2018Deeper} hypothesize that this alignment of communities and node labels may be the main reason why GNNs achieve state-of-the-art performance on the classification task. In this paper we aim to experimentally test this hypothesis on six datasets from different domains. 
%\dhe{has this paper shown this already? if yes, why do we perform our analysis? are there some questions, which remained unanswered in that paper? if yes, we need to discuss them and argue that we are trying to address those unanswered questions with our work.}\hussain{the paper mentions this as a premise, I think we start with this premise as well to investigate more when GNNs don't work, and the unanswered question for us is `where are (not) GNNs applicable?' Is it enough to point out that the other case is not well-studied?}.

In the other case, which is typically ignored in literature, the cluster assumption does not hold, and a community could possibly have a variety of labels.
The feature propagation between nodes of the same community would therefore result in feature smoothing for nodes with different labels.
This eventually makes the classification task harder since representation similarity does not imply label similarity in this case.

In summary, in this paper we set out to quantify the label-community correlation and how this correlation is related to the performance of GNNs on semi-supervised classification task on graphs.

%Aiming to quantify the cluster assumption on a community level, and assess the applicability of GNNs on a given labeled graph, we utilize the following metric.

\section{Methods and Experiments}

%\para{Label-community correlation.}
%\label{sec:information-theory}
We start by quantifying how much information node's community reveals about its label.
For a labeled graph, let $L$ be a random variable taking values in the set of labels $\mathcal{L}$, i.e., $L(u)$ is the label of node $u \in V$.
Assuming the graph is partitioned into a set of disjoint communities $\mathcal{C}$, we define another random variable $C$ taking values in $\mathcal{C}$, i.e., $C(u)$ is the community of node $u \in V$.

To measure how much the (fraction of) uncertainty about $L$ is reduced knowing $C$, we use the uncertainty coefficient~\cite{press1992numerical} of $L$ given $C$.
This coefficient can be written as $U(L|C)=\frac{I(L;C)}{H(L)} \in [0,1]$, where $H(L)$ is the entropy of  $L$, and $I(L;C)$ is the mutual information between $L$ and $C$.

When the uncertainty coefficient equals $1$, all nodes within each community share the same label, and thus knowing the node's community means also that we know the node's label. On the other hand, when the uncertainty coefficient is $0$, the label distribution is identical in all communities, so knowing the community of a node does not contribute to knowing its label. In general, the higher the eliminated uncertainty about the labels when knowing communities is (i.e., the closer $U(L|C)$ is to $1$), the more likely it is that the cluster assumption holds, and thus GNNs can exploit the graph structure, and vice versa.%
% As this coefficient takes values in $[0,1]$ and is independent of the number of labels and communities, we can compare its value for different graphs.

%\para{Uncertainty coefficient and the cluster assumption.}
%Assuming that a graph exhibits community structure, the cluster assumption would translate into the following: \textit{`nodes within the same community are more likely to have the same label'.}
%In case this assumption holds, that statement would imply that knowing the community of a node should eliminate some uncertainty about its label.
%This relationship between the community and the label maps to the description of $U(L|C)$ above.
%The higher this eliminated uncertainty is (i.e., the closer $U(L|C)$ is to $1$), the more likely it is that the cluster assumption holds, and thus GNNs can exploit the graph structure, and vice versa.% \dhe{Explain also the numerical link to the uncertainty coefficient.}% and increase the accuracy.
% Empirically, we have shown this correlation in Table~\ref{tab:label-community}.
%Thus, we interpret the uncertainty coefficient as an indicator to whether the cluster assumption holds in the graph, and hence whether GNNs are applicable or not on a certain graph.


==> conclusion.tex <==

\section{Conclusion}

In this work, we analyzed the impact of community structures in graphs on the performance of GNNs in semi-supervised node classification, with the goal of uncovering limitations imposed by such structures.
By conducting ablation studies on the given graphs, we showed that GNNs outperform a given baseline on this task in case the cluster assumption holds. Otherwise, GNNs cannot effectively exploit the graph structure for label prediction.
Additionally, we show an analysis on the relation between labels and graph communities. With our analysis, we suggest that when community information does not contribute to label prediction, it is not advisable to use such GNNs.
In particular, we show that the uncertainty coefficient of node labels knowing their communities can indicate whether the cluster assumption holds.
We further formalize a guideline to select where to apply GNNs based on community-label correlation.
% This finding can serve as an initial guideline to select where to apply GNNs based on the correlation between labels and graph structure.
% We also show that hubs are key transmitters which propagate features quickly across the graph. We further analyze the difference between the role of global hubs and local hubs using synthetic graphs. We find that, \textit{when the cluster assumption holds}, local hubs contribute to feature smoothing and simplify the classification task, while global hubs contribute to feature oversmoothing and hinder the classification task.
% As an additional guideline, one should aim to identify global hubs before applying GNNs to lessen the risk of oversmoothing and impairment of the classification performance.
Our work serves as a contributing factor to intrinsic validation of the applicability of GNN models.
Future work can also investigate the effect of other graph structural properties such as edge directionality, degree distribution and graph assortativity on the GNN performance.


==> discussion.tex <==

% \section{In-depth analysis}
% \rkern{Since this is not exactly a discussion, could we rename it s/t like: in-depth analysis?}
% \subsection{Community impact}
% The results show that GNNs could consistently outperform the feature-only baseline on citation graphs but not on the other two datasets.
% % \hussain{I'm going with the word 'consistently' as the behavior wasn't consistent on twitter, and to have twitter on the side with webkb or at least somewhere in between, also, the significance test showed that when the baseline is outperformed on Twitter, it is surprisingly significantly outperformed! so I couldn't go with 'significantly outperform' here}.
% Besides, we see a contrast between the performance on SBM graphs of the citation datasets and the other two datasets. As this ablation model preserves community structure, the observations suggest a dependency of the citation datasets on communities whereas these structures could worsen the predictions in the other two datasets.
% In other words, the cluster assumption holds in the citation graphs and to a smaller degree in the Twitter dataset while it does not hold in WebKB.
% To support this linking to the cluster assumption, we further analyze the relationship between communities and labels in each of these datasets.
% % To interpret the difference in results from one dataset to another, we perform additional analysis of the given graphs.
% In the next analysis, we aim to quantify how much knowing a node's community reveals about its label.



% \hussain{uncertainty coefficient U(L|C): having the community information available reduces the probability that we will make an error predicting the label by U(L|C) - interpretation taken from a YT vid}.

% The lower the value of this metric is, the closer is the label distributions within communities to the overall label distribution, and hence the less information is revealed about the labels by knowing the community.
% \hussain{add an explanation of what this metric actually translates to in words, i.e., the less it is, the closer the label distributions within communities to the overall label distribution}

% Another simple metric we report is the ratio of edges which connect nodes of the same class to all the edges in the graph. Both metrics are shown in Table~\ref{tab:label-community} for each dataset.

% \begin{table}[b]
%     \centering
%     % hey Roman... hello there!
%     % we've finished the intro, and handled the comments, there is still one comment about the semi supervised learning, if you could just see whether it's good now (only this comment if you will) - ok, on my way Thanks!
%     \caption{The correlation between our observations and the uncertainty coefficient. We see that the lower $U(L|C)$ is, the less probably are GNNs to outperform the feature-only baseline, and the less likely are communities to preserve accuracy.
%     %\rkern{not always sounds strange, maybe not consistently, or exact number or percentage <10\%}
%     %\hussain{remove intra-class edge ratio unless it makes sense to show that our suggested metric correlates better with the results}
%     }
%     \label{tab:label-community}
%     \begin{tabular}{cHcccc}
%         \toprule
%         \thead{Dataset} & \thead{Intra-class\\edge ratio} & \thead{$U(L|C)$} & \thead{Outperformed baseline \\ on original graphs} & \thead{SBM preserved\\most accuracy} \\
%         \midrule
%         CORA-ML & 0.804 & 0.586 & \checkmark & \checkmark\\
%         CiteSeer & 0.736 & 0.488 & \checkmark & \checkmark \\
%         PubMed & 0.802 & 0.404 & \checkmark & \checkmark \\
%         CORA-Full & 0.567 & 0.442 & \checkmark & \checkmark \\
%         Twitter & 0.707 & 0.289  & $2/3$ cases & $2/3$ cases \\
%         WebKB & 0.138 & 0.080 & $\times$ &  $\times$ \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% look at table 3
% high U for citations <-> cols3,4
% slightly lower U for twitter <-> cols3,4
% much lower U for WebKB <-> cols3,4
% U(L|C) indicates whether cluster assumption holds

% Table~\ref{tab:label-community} compares our observations to the uncertainty coefficient.




% Comparing this to the description of $U(L|C)$, 
% On WebKB and Twitter, the GNNs could not consistently outperform the feature-only baseline. \rkern{Maybe rephrase the following sentence, not clear to me}The correlation we see is between the uncertainty coefficient and the ability to significantly outperform the feature-only baseline: the lower the coefficient is, the less likely are GNNs to exploit the graph structure and improve over the feature-only baseline performance.
% We notice from Table~\ref{tab:label-community} that the coefficient is relatively high for the datasets where the SBM graphs preserved more accuracy than the other ablation models, i.e., citation graphs.
% Meanwhile, the coefficient is particularly small for the WebKB dataset where the SBM graphs had the lowest accuracy.
% In Twitter's case, the performance drop on SBM graphs was moderate comparing to other ablations \elex{add the numbers in percentages}, which is again reflected in the coefficient value that is relatively moderate for Twitter compared to the other datasets.

% \subsection{Hubs impact}
% % The results show that random graphs could preserve more accuracy than the CM graphs.
% % Our interpretation for this, as the ablation suggests, is the existence of hubs in CM graphs.
% % Since communities are eliminated in both cases, most propagation of features across the graph will be noisy, i.e., passing correct messages to the wrong entities.
% % With no particular community structure, the existence of hubs can cause a faster propagation of noise.
% % \rkern{again, I am not sold on the notion of noise propagation, but I like the "barrier" argument below}
% % This suggests that noise propagation will be more contained in the random graphs than in CM graphs (because of hubs), hence a lower performance on CM graphs.

% % The results show that random graphs could preserve more accuracy than the CM graphs.
% % Since communities are eliminated in both cases, hubs are most likely accelerating the propagation of features between nodes of different labels.
% % In contrast to hubs, community structures provide barriers for propagation, hence slowing down both true and noisy feature propagation~\cite{hasani2018consensus} as shown for SBM graphs.
% Looking at Figure~\ref{fig:results}, the absence of hubs in SBM graphs caused a performance drop when compared to the original graphs. However, the absence of hubs in random networks caused a performance increase comparing to CM networks.
% This brings two types of hubs to mind \textit{assuming the cluster assumption holds}:
% \begin{itemize}
%     \item \textbf{local hubs}, which connect nodes within the same community, and hence most likely with the same label
%     \item and \textbf{global hubs}, which connect nodes from different communities, hence most likely with different labels.
% \end{itemize}
% % When the cluster assumption holds, these types also translate to local (intra-community) and global (inter-community) hubs.
% To study the effect of these types of hubs on GNNs, we carry out the following experiment.

% \para{Local vs. global hubs.}
% We aim to create a synthetic graph with original features and labels, so we chose a set of nodes from the WebKB dataset along with their assigned features and labels. For more details on the graph construction, refer to Appendix~\ref{app:hubs}.
% Using the stochastic block model, we build a synthetic graph from this set of nodes where nodes with the same label are more likely to connect to each other, i.e., the cluster assumption holds.
% This results in a graph with $5$ main communities, i.e., one community for each label.
% % In total, we create $1,465$ edges in this graph.
% Since this graph is built using the stochastic block model, the degree distribution is not skewed, and there are no major hubs~\cite{karrer2011stochastic}.
% We compare GNNs performance on this graph after injecting local hubs and  global hubs.
% % \hussain{@Denis, I've edited the experiment to have a close number of added edges for local and global cases in total (it was 2000 new edges for global before) I thought that would make the comparison more fair}
% \begin{enumerate}[label=(\alph*)]
%     \item For local hubs, we pick a small set of nodes in each community and add edges between them and other nodes in the same community, i.e., adding shortcuts within communities.
%     %This results in the addition of $792$ new edges.
%     % 2257 in total
%     \item For global hubs, we randomly pick a small set of nodes from the graph, and add edges between these nodes and other nodes in the entire graph, i.e., adding shortcuts between communities.
%     % This results in the addition of $732$ new edges. \dhe{how these other nodes are picked? why exactly this number of nodes?}\hussain{i explain that in the appendix, should I leave the numbers here? or can I mention that we're adding similar number of edges?}
%     % 2197 in total
% \end{enumerate}
% The total number of added edges is similar in the two cases, cf. Appendix~\ref{app:hubs}.
% % \hussain{injecting the hubs this way is probably favoring the local ones, will verify and modify accordingly}

% % the following could be moved to the appendix
% % We take WebKB, we build a stochastic matrix based on ground truth labels, we build a graph using the stochastic block model -> no-hubs graph
% % We take the no-hubs graph. For each label, we select $2\%$ of its nodes at random to be \textit{local} hubs we link each of these hubs to a random set of nodes of the same label, whose size is $20\%$ of the number of nodes with this label. This is a graph with local hubs.
% % We take this no-hubs graph, we select $2\%$ of its nodes at random to be \textit{global} hubs, we link each of these hubs to a random set of nodes, whose size is $20\%$ of the graph size. This is a graph with global hubs.

% Figure~\ref{fig:local-vs-global} shows a comparison between the local and global hubs.
% We notice that adding local hubs improves accuracy for the studied GNNs.
% Since the cluster assumption holds, adding these shortcuts within a community increases its connectivity and hence accelerates feature smoothing.
% Meanwhile, adding global hubs mostly decreases the accuracy.
% With the cluster assumption in mind as well, a global hub adds shortcuts between different communities. Therefore these hubs accelerate oversmoothing and result in worse classification accuracy.

% This analysis provides an interpretation to the role of both types of hubs on the propagation in GNNs.
% Particularly, this analysis supports the following hypothesis: when the cluster assumption holds, global hubs accelerate propagation between nodes with different labels causing oversmoothing.
% However, local hubs accelerate the propagation of true features within communities causing normal feature smoothing. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/discussion/local-vs-global-hubs.pdf}
%     \caption{Comparison between having no hubs, adding local hubs and adding global hubs. For each violin plot, the white dot represents the median accuracy. The horizontal dashed red line represents the median performance of the feature-only baseline. We see that adding local hubs increases the accuracy, while adding global hubs decreases it.}
%     \label{fig:local-vs-global}
% \end{figure}

% % In order to compare this value between two datasets, we need to normalize it by its label distribution.

% % \begin{figure}
% % \centering
% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/cora.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/citeseer.pdf}

% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/pubmed.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/cora_full.pdf}

% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/twitter.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/community_information_gain/webkb.pdf}
% % \caption{Relation between ground truth labels and communities detected via Louvain method for each dataset. The relative information gain is shown in the figure title. We notice that for WebKB, the knowledge of the community does not help guessing the label.}

% % \end{figure}



% % \begin{figure}
% % \centering
% % \includegraphics[width=0.49\textwidth]{figures/label_transition/cora.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/label_transition/citeseer.pdf}

% % \includegraphics[width=0.49\textwidth]{figures/label_transition/pubmed.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/label_transition/cora_full.pdf}

% % \includegraphics[width=0.49\textwidth]{figures/label_transition/twitter.pdf}
% % \includegraphics[width=0.49\textwidth]{figures/label_transition/webkb.pdf}
% % \caption{Transition stochastic matrix between nodes grouped on labels. Each cell represents the edge density between two groups of nodes (e.g. from nodes with label 'student' to nodes with label 'course' in WebKB). The density in cell $(L_1,L_2)$ is the number of existing edges from nodes with label $L_1$ to nodes with label $L_2$ divided by the maximum possible number of edges from $L_1$ to $L_2$, i.e., $|L_1| \times |L_2| $. All datasets except WebKB show a high density on the main diagonal, indicating the strong connection between nodes of the same type.}
% % \end{figure}



==> experiments.tex <==
% \section{Experimental setup}

% \para{Feature-only baseline.}
% Aiming for a simple baseline, we use logistic regression to classify nodes given node feature vectors.
% This baseline takes only the node feature information and completely ignores the graph structure.
% We compare this feature-only baseline to GNN performances on each of the ablation models.
% The aim of using such a baseline is to spot when graph structure causes GNNs to propagate noise, i.e., propagating true features to wrong entities.
%\rkern{Nitpicking: graph structure might still contribute additional knowledge, but the GNN might be unable to use it}
%\dhe{explain baseline before you explain the gnns. you do not a subsection for such a short section.}

% \subsection{Graph neural network models\hussain{summarize and mix with the above}}
% In our experiments, we study three GNN architectures which are widely used for semi-supervised classification on graphs:

% % \begin{itemize}
%     \para{Graph Convolutional Network (GCN)}~\cite{gcn}, introduced as a linear approximation of spectral graph convolution~\cite{Hammond2011}. It was shown to be effective on semi-supervised classification while being comparatively simple~\cite{shchur2018pitfalls}.
    
    
%     \para{GraphSAGE}~\cite{graphsage} was introduced to handle inductive representation learning. However, it can also be applied in transductive settings such as ours. GraphSAGE uses neighborhood sampling and then applies aggregation. In our experiments, we use the simple yet effective~\cite{shchur2018pitfalls} variant with mean-based aggregator.
    
%     \para{Graph Attention Network (GAT)}~\cite{gat}
%     %is considered to be the state of the art in graph representation learning~\cite{wang2019improving}\hussain{self-note: maybe find a better opener, and remove this one}.
%      proposes attention mechanism allowing each node to assign different weights to its neighbors in order to treat neighbors differently during aggregation.
%     Despite their effectiveness, introducing these attention weights as model parameters increases model complexity.
    
%     \para{Relational Graph Convolutional Network (RGCN)}~\cite{rgcn2017kipf} is designed to handle knowledge graphs and is able to exploit asymmetry in relations.
% Since our datasets (see Section~\ref{sec:datasets}) feature only homogeneous graphs (not knowledge graphs), we only have one type for an edge in one direction.
% Therefore, RGCN reduces to two relation types for each existing directed edge: one relation in the direction of the edge and another in the inverse direction.
% For example, the edge from node $u_1$ to node $u_2$ is represented by both \textit{<$u_1$,~relation,~$u_2$>} and \textit{<$u_2$,~inverse~relation,~$u_1$>}.

% \tdu{try to rewrite this slightly so that this last bracket is not broken in two lines (it's broken when you remove my comment), also for consistency decide on the naming conventions used throughout the text (edge vs link, graph vs network, etc.)} \hussain{1. done with a cheap trick, will verify whether it looks ok when in case we modified content.} \hussain{2. converted link to edge and network to graph (except for the term complex networks), also not sure about saying web graphs, citation graphs or retweet graphs, I mean they are right but sound strange to me}
% \dhe{we could move this description in the bullet point, that is exactly a kind of extension that i meant. maybe to avoid losing too much space we could change the bullet points to textbfs.}
% \dhe{generally, i think that we should explain these approaches with more details. just try to extend each description with two or three additional sentences.}



% Here, we also use the same splitting criteria (explained later) with the same number of labelled examples in the training and validation sets.

% \subsection{Datasets\hussain{summarize}}
% \label{sec:datasets}
% % \rkern{Very nice section intro!}
% To provide a better understanding of the roles of the studied structures, we aim for a diverse selection of datasets with respect to
% \begin{enumerate*}[label=(\alph*)]
%     \item domain, e.g., citation, social and web graphs,
%     \item structure, e.g., directed acyclic vs. cyclic,
%     \item and correlations between community and labels, i.e., whether nodes of the same community tend to share the same label. 
% \end{enumerate*}
% With this in mind, we use the following set of datasets.
% \dhe{yes, start the dataset description with the argumentation why we selected these datasets. before explaining the individual datasets provide general arguments what we wanted to achieve with this selection of datasets, i.e., we wanted domain diversity, structural diversity (cyclic vs. acyclic), diverse community structures, diverse correlations between community and labels, social vs. colloboration vs. information graph, etc. then explain how our selection satisfies these critearia and only then explain the datasets in more details.}

% \begin{table}[b]
% \caption{Dataset statistics after preprocessing (similar to Shchur et al.~\cite{shchur2018pitfalls}). We use 20 and 30 examples per label for training and validation respectively for all datasets except WebKb where we use 10 and 15 respectively. The label rate represents the ratio of nodes in the \textit{training} set. The edge density is the number of existing undirected edges divided by the maximum possible number of undirected edges (ignoring self-loops).}
% \label{tab:datasets}
% \centering
% \begin{tabular}{lrrrrrr}

% \toprule
% Dataset & Labels & Features & Nodes & Edges & Edge density & Label rate \\
% \midrule
% CORA-ML & 7 & 1,433 & 2,485 & 5,209 & 0.0017 & 0.0563 \\
% CiteSeer & 6 & 3,703 & 2,110 & 3,705 & 0.0017 & 0.0569 \\
% PubMed & 3 & 500 & 19,717 & 44,335 & 0.0002 & 0.0030 \\
% CORA-Full & 67 & 8,710 & 18,703 & 64,259 & 0.0004 & 0.0716 \\
% Twitter & 2 & 215 & 2,134 & 7,040 & 0.0031 & 0.0187 \\
% WebKB & 5 & 1,703 & 859 & 1,516 & 0.0041 & 0.0582 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \para{Citation graphs.}
% We use four citation graph datasets: CORA-ML~\cite{sen2008collective}, CiteSeer~\cite{sen2008collective}, PubMed~\cite{pubmed} and CORA-Full~\cite{corafull}, where nodes are paper, and edges are citations.
% In these graphs, the feature vector of a node represents a bag of (dictionary) words of the paper, and the label of a node represents the topic of the paper.
% These graphs feature a directed acyclic structure as opposed to the next two graphs which include cycles.
% % "Each publication in the dataset is described by a 0/1-valued word vector indicating the absence/presence of the corresponding word from the dictionary" - source: https://linqs.soe.ucsc.edu/data


% \para{Retweet graph.}
% `Hateful users on Twitter'~\cite{twitter} is a retweet graph where nodes are Twitter users, and edges exist between two users if one of them has retweeted the other.
% The class of each user is a binary indicator to whether the user is 'hateful' or 'normal'.
% In the original dataset, we have $100,000$ users with approximately $2,200,000$ edges. Only $4,971$ users are labeled as 'hateful' or 'normal' and the rest are unlabeled.
% We first consider only the labeled nodes, then we select the largest weakly connected component of these nodes.
% %This leaves us with $2,134$ nodes and $7,040$ edges.
% Then we apply cleaning~\footnote{We plan to release a code to reproduce the dataset from the original one.} to the feature vectors of nodes same as in~\cite{Tiao2019}, i.e., removing graph-based features and GloVe features. 
% % We end up with feature vectors of length $215$ \hussain{verify}.


% \para{Web graph.}
% The WebKB dataset~\cite{webkb} is a web graph where each node is a web page and the edges represent hyperlinks between these web pages.
% These web pages are collected from the websites of four universities.
% The classes represent the type of the web page, being either course, faculty, project, staff or student.
% The feature vector of a node represents a binary bag of words of the web page content (ignoring words with less than 10 occurrences). 

% \para{Common graph preprocessing.}
% While the original graphs are directed, we treated them as undirected by ignoring the edge direction (as is the case for most previous works~\cite{gcn,graphsage,shchur2018pitfalls}).
% % For RGCN, which has an asymmetric architecture, we keep the edge directionality.
% All of these graphs are preprocessed in a similar manner as Shchur et al.~\cite{shchur2018pitfalls}, i.e., removing nodes with rare labels and selecting the largest weakly connected component except in WebKB where we take 4 connected components representing 4 universities.

% \para{Why could these datasets be interesting for this problem?}
% \label{sec:dataset-interest}
% The label of a node in a \textbf{citation graph} represents the topic of the paper. Citations are expected to be denser among papers with similar topics than they would be between papers of different topics. For example, a publication about natural language processing would be more likely to cite other natural language processing papers than human-computer interaction papers. Therefore, one could intuitively expect that papers within the same graph community tend to have the same label.
% In the \textbf{Twitter} dataset, one could not easily assume the presence or the absence of a correlation between communities and labels (hateful or normal). In other words, we do not know whether hateful users typically form communities as this highly depends on the dataset itself, i.e., the environment these users were in during that time.
% For \textbf{WebKB} dataset, one cannot intuitively assume that nodes within a graph community are expected to share a label.
% For example, a web page of a staff member could be more likely to link to projects on which this staff member is working than to other staff members' web pages.
% Based on these intuitions, we think that this set of graphs is sufficiently diverse concerning community impact on label prediction (more support to our assumption in Section~\ref{sec:information-theory}).



% \subsection{Network analysis}
% \hussain{explain the knowledge we collect about the networks, e.g., community information gain, label transition matrix, intra-class edge ratio, degree distributions, ...}


% \subsection{Hyperparameter search\hussain{remove}} 
% %hyperparams
% We perform hyperparameter search for the considered GNNs using a similar grid search to the one in~\cite{shchur2018pitfalls}, but on a smaller space of hyperparameters.
% We evaluate the hyperparameter settings for each GNN on CORA-ML and we select the model that maximizes the validation accuracy on this dataset to apply it to all others (as in~\cite{gat}).
% % \dhe{what is arguemnt for optimizing only on cora-ml and not on each dataset individually?}\hussain{this has been done in two works on these datasets, can't I just mention these works?}
% However, GAT is an exception to this since the authors of that work~\cite{gat} recommended a different setting for PubMed. Therefore, we perform a grid search for GAT on PubMed, and used the selected setting for PubMed as well as Cora-Full which is of a similar size and nature.
% This hyperparameter search is performed on the original graphs, but the selected settings are applied to all the ablation models explained in Section~\ref{sec:ablation}.
% More details on hyperparameters setting in Appendix~\ref{app:hyper}.


% \subsection{Evaluation setup\hussain{summarize}}
% % explaining how a single split looks like
% Following the train/validation/test split strategy as in~\cite{shchur2018pitfalls}, each random split consists of $50$ labeled examples per class ($20$ for training and $30$ for validation) and the rest are considered test examples.
% This applies to all of our datasets except WebKB where we use $10$ training examples and $15$ validation examples per class due to the fewer number of nodes.

% % splits on original graphs and baselines
% To evaluate the GNN models on the original graphs, we follow the evaluation setup as conducted in~\cite{shchur2018pitfalls} by having $100$ random splits and $20$ random model initializations for each split.
% The same process is carried out to evaluate the feature-only baseline (logistic regression) model.
% The evaluation is slightly different for the ablation studies (SBM, CM and random graphs) as they include an additional level of randomization.
% For a given dataset, we generate SBM, CM and random graphs with $10$ different random seeds, which results in $10$ SBM graphs, $10$ CM graphs and $10$ random graphs.
% The evaluation on each of these generated graphs is carried out through $50$ different random splits and $10$ different random initializations.
% % For the completely random graphs, we generate a single random regular graph for each dataset. Then we perform the evaluation with $100$ random splits $\times~20$ random initializations.
% % \hussain{verify this and maybe generate 10 random graphs and make the evaluations similar to SBM and CM}
% % conclusion of splits on original graphs and baselines

% As a result, the reported accuracy for a GNN architecture on the original graph is presented for $2,000$ trainings of the GNN.
% Meanwhile, the reported accuracy of a GNN architecture on one of the ablation models (SBM, CM or random graphs) is presented for training the GNN $5,000$ times, i.e., $10$ randomly generated graphs $\times$ $50$ random splits $\times$ $10$ random model initializations.



==> introduction.tex <==
\section{Introduction}

%\para{Motivation.} 
Many real-world systems are modeled as complex networks, which are defined as graphs with complex structural features that cannot be observed in random graphs~\cite{kim2008complex}.
The existence of such features governs different processes and interactions between nodes in the graph.
In particular, community structures are often found in empirical real-world complex networks. These structures have a major impact on information propagation across graphs~\cite{barabasi2013network} as they provide barriers for propagation~\cite{hasani2018consensus}.
The process of information propagation forms the basis for many studied applications on graphs.
Among these applications, graph-based semi-supervised learning~\cite{gcn,zhu2003semi} is widely studied and particularly of interest.
Graph-based semi-supervised learning aims to exploit graph structure in order to learn with very few labeled examples~\cite{Li2018Deeper}.
In recent years, state-of-the-art methods for this task have predominantly been graph neural networks (GNNs)~\cite{shchur2018pitfalls}. 

\para{Problem.} Despite the outstanding results of GNNs on this and similar tasks, there is still a limited understanding of their abilities and constraints, which hinders further progress in the field~\cite{Loukas2020What,Xu2019How}. To the best of our knowledge, there is a lack of research on how common graph structures, such as communities, impact the learning process of GNNs.

\para{The present work.}
We are particularly interested in the influence of community structure on the performance of GNNs in semi-supervised node classification.
%Considering their ubiquity and their impact on information propagation, communities appear as a promising starting point for such a study.
From a practical perspective, we set out to provide a set of guidelines on the applicability of GNNs based on the relationships between communities and target labels.
To that end, we design an evaluation strategy based on an ablation study on multiple graph datasets with varying characteristics in order to study the behaviour of GNNs.
Using this evaluation strategy we compare the performance of GNNs on six public graph datasets to a simple feature-based baseline (i.e., logistic regression) which ignores the graph structure.

To gain a deeper understanding on the role of communities, we compare the change in performance of GNNs after (i) eliminating community structures while keeping the degree distribution, (ii) keeping the community structure while using a binomial degree distribution, and (iii) eliminating both.
Finally, we link the evaluation results on the ablation models to the relationship between communities and labels in each dataset.
To achieve this, we compute the uncertainty coefficient~\cite{press1992numerical} of labels with respect to communities, before and after applying community perturbations.

\para{Findings.}
Our results show that GNNs are able to successfully exploit the graph structure and outperform the feature-based baseline only when communities correlate with the node labels, which is known in the literature as the cluster assumption~\cite{chapelle2009semi}.
If this assumption fails, GNNs propagate noisy features across the graph and are unable to outperform the feature-based baseline.

\para{Contributions.}
With our work, we highlight the limitations that community structures can impose on GNNs.
% We additionally perform further analysis on these datasets to provide interpretations for the impact of communities. \dhe{rewrite this sentence and give a concrete example of what we are doing}
We additionally show that the proposed uncertainty coefficient measure helps predicting the applicability of GNNs on semi-supervised learning.
We argue that this measure can set a guideline to decide whether to use GNNs on a certain semi-supervised learning task, given the relationship between communities and labels.



% \hussain{rest of intro to be removed}

% % Scope
% Graph neural networks (GNNs) have been widely used for various applications on graphs data~\cite{wu2019comprehensive}.
% %\cite{gcn,graphsage,Li2016gated,Klicpera2019predict,rgcn2017kipf}.
% In particular, GNNs have significantly improved the state of the art for the semi-supervised node classification task on graphs~\cite{gcn,gat}.
% % Motivation
% In spite of these promising results of GNNs on this and similar tasks, we as a research community still lack a deeper understanding of their abilities and limitations, which is hindering further progress in the field. \elex{motivation needs to be more specific and tailored towards your work} \hussain{I've mentioned some more specific things after the related work paragraph}
% % Related work
% This lack of understanding has inspired few works aiming at a thorough characterization of GNNs in theory and in practice.
% Notable examples include the studies on the expressive power of GNNs~\cite{Morris2019Weisfeiler}, the classes of problems they can and cannot solve~\cite{Loukas2020What}, the local structures they can and cannot distinguish~\cite{Xu2019How}, and the role of their architecture (e.g., number of convolutional layers) when used for semi-supervised learning~\cite{Li2018Deeper}.
% % Gap
% However, limited work has been conducted to study the relationship between common graph structures and the behavior of GNNs.
% Two phenomena particularly common in complex networks are community structure and hub nodes~\cite{barabasi2013network}.
% The existence of community structure and hub nodes has a major impact on information propagation in graphs~\cite{kitsak2010identification}, which directly concerns the propagation mechanism of GNNs.

% \noindent\textbf{The present work.} We study the behavior of GNNs in the presence and the absence of these two graph structures, i.e., communities and hubs.
% % \noindent\textbf{The present work.} \tdu{"This work" as a paragraph title feels a bit awkward, not sure if you even need it, also this first sentence is slightly awkward and would rewrite it} We study the effect of the presence and absence of common graph structures on GNNs. 
% % In particular, we study the impact of community structure and graph hubs since they are two common phenomena~\cite{barabasi2013network,albert2002statistical} which have major impact on the diffusion of information across the graph~\cite{kitsak2010identification}. 
% \elex{that needs to be better motivated. in the paragraph before you motivate the work in a generic way so the reader wonders why now suddenly you talk about information diffusion} \hussain{explained the gap after the related work, and then started with this work, do you think I should be specific about the structures even earlier in this section?}
% % \noindent\textbf{This work.} Currently, the impact of graph structures, which are typically observed in real graphs, on the learning process of GNNs is not well studied.\hussain{rewrite}
% % \hussain{For example, the asymmetric relationships between nodes in directed graphs are typically not well exploited by GNNs: a little out of scope though}. 
% % Our interest
% % In particular, community structure and graph hubs are two common phenomena~\cite{barabasi2013network,albert2002statistical} which have major impact on the diffusion of information across the graph~\hussain{refs}.
% % Goal
% With this work, we aim to experimentally uncover \elex{we aim to experimentally uncover - avoid ing forms} the role of community structure and hubs in graphs on the performance of GNNs in the context of semi-supervised node classification. From the practical perspective, we set out to provide a set of simple guidelines on the applicability of GNNs based on the relationship between the target labels and common structural patterns in graphs such as communities and hubs.
% % We further analyze the role of hubs by looking at them as local (intra-community) hubs and global (inter-community) hubs.
% % \dhe{here you can give references to various applications where gnns are used, thus showing their importance and role in classification tasks on graphs. then make an argument that although they work well we know little about why their work that well. you can also mention the situation with directed/undirected. then you can say that we also do not know much about how common structures in graphs such as communities and hubs impact the performance on gnns. and that with this work we aim at uncovering this relation and providing a set of simple guidelines for how to apply gnns in presence of various structural properties in graphs.}
% % How?
% % We use a selection of six public graph datasets which show different strength of correlation between node labels and communities.
% To that end, we first compare the performance of GNNs on six public graph datasets to a simple feature-based baseline.
% Then, using a set of ablation studies on these datasets, we compare the performance drop of GNNs after eliminating (i) community structures, (ii) degree sequences, or (iii) both.
% We then interpret the difference in GNNs behavior on each ablation model.
% To investigate the impact of communities, we first study the correlation between communities and labels in each dataset, and then analyze the relation between this correlation and the performance achieved by GNNs on ablation models.
% % We also show that the nature of how labels are distributed across the graph indicates whether GNNs can exploit the graph structure.
% % We also show that this correlation can tell whether GNNs are able to exploit the original graph structure to improve on the performance of a baseline which only considers node features and completely ignores the graph structure. \dhe{do not understand this completely but maybe we can omit this sentence all together.}
% We further study the role of hubs, by conducting a similar evaluation on a synthetic graph where we artificially inject hubs of two types: local (intra-community) hubs and global (inter-community) hubs.


% % Findings
% Our results show that GNNs are only able to exploit the graph structure, improving over the feature-based baseline, when node communities correlate with their labels, i.e., when the cluster assumption holds~\cite{chapelle2009semi}.
% Otherwise GNNs spread noise across the graph and are unable to outperform even this simple baseline.
% These observations also reflect the diversity in our selection of datasets with respect to the correlation between node communities and labels.
% Moreover, we find that hubs are the main transmitters of both label signal and noise. In particular, when the cluster assumption holds, local hubs propagate feature information correctly whereas global hubs mainly spread noise, i.e., passing correct feature information to the wrong entities.
% \elex{if there are differences between datasets, mention them here. } \hussain{explained above now, please check}

% % Contribution
% With our work, we highlight limitations graph structures can impose on GNNs.
% We also provide an interpretation to the roles of communities and hubs on GNNs performance, supported by empirical evaluation.
% Our interpretations constitute a set of simple guidelines indicating when GNNs are applicable for semi-supervised learning in terms of (a) the relation between labels and community structure and (b) the existence of local and/or global hubs.
% % Impact
% We believe that our work can form a basis for \elex{that sounds rather weak}\hussain{corrected, check pls} the development of GNN architectures, which can adapt to a variety of graph structures existing in real graphs.
% % Future work can also study the impact of other common graph structures on the performance of GNNs on various graph-related machine learning tasks. \elex{future work should go into last section}





==> results.tex <==
\subsection{Results}

We summarize the evaluation results of the GNN models with respect to accuracy for the original graph and its corresponding ablation models in Figure~\ref{fig:results}.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy1-2.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy3-4.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy5-6.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy-violin1-2.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy-violin3-4.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/ablation/accuracy-violin5-6.pdf}
    \includegraphics[width=0.95\textwidth]{accuracy-prelim1-3.eps}
    \includegraphics[width=0.95\textwidth]{accuracy-prelim4-6.eps}
    
    % \includegraphics[width=\textwidth]{figures/ablation/accuracy1-3.pdf}
    % \includegraphics[width=\textwidth]{figures/ablation/accuracy4-6.pdf}
    % \includegraphics[width=\textwidth]{figures/ablation/accuracy-violin1-3.pdf}
    % \includegraphics[width=\textwidth]{figures/ablation/accuracy-violin4-6.pdf}
    \caption{The accuracy of GNNs on the original graph and the ablation models of each dataset.
    % For each box plot, the white dot represents the median accuracy.
    The red dashed line represents the median accuracy of the feature-only baseline.
    The performance on the original graphs is generally higher than that of the baseline except for WebKB.
    On citation graphs, the baseline is clearly outperformed on the original graphs, and eliminating communities (CM graphs) results in a much higher accuracy drop than eliminating the degree sequence (SBM graphs).
    This is not the case for the other two datasets where the baseline is not always outperformed on the original graphs, and the drop in performance on SBM networks is substantial. This highlights the positive impact of communities on citation datasets and its negative impact on WebKB. %, and could reflect the correlation between communities and labels that is different in each dataset, i.e., whether the cluster assumption holds.
    The uncertainty coefficient is the highest for the three datasets in the top row and the lowest for WebKB providing a potential explanation for the low GNN performance on this dataset.
    % Preserving the degree distribution (CM graphs) surprisingly causes a larger performance drop than eliminating both the communities and degree distribution. This highlights the role of \textit{hubs as main spreaders which can potentially cause oversmoothing}\hussain{how to rephrase that? does the observation actually hold?}.
    }
    \label{fig:results}
\end{figure}

\para{Could GNNs outperform the simple baseline?} 
%\dhe{general comment for description of results: first, describe what we see, i.e. what are our results. second, describe what does it mean. third, discuss shortly implications or our explanations of the results. in this specific case you need first to describe which of the approaches beat the baseline etc. only then you should talk about the significance of the results and how we compute the significance.} 
Comparing the performance of GNNs on the original graphs with the feature-only baseline, all GNN models clearly outperform the baseline on the citation datasets. For the Twitter dataset however, GAT could not outperform the baseline, while GCN and GraphSAGE outperformed it only by a small margin. 
This is more prominent for WebKB where none of the GNNs outperforms the baseline on the original graph.
% . These observations are even more pronounced on the WebKB dataset, where the performance overlap is more obvious, and more importantly, all GNNs could not outperform the baseline on the original graph.
This suggests that for the two latter datasets, the graph structure is either irrelevant to the learning process or is even hindering it. To test the statistical significance for each approach on each dataset against the corresponding baseline, we compute the non-parametric \textit{Mann-Whitney U test} for unpaired data with the significance level $\alpha=0.01$ (Bonferroni corrected).
The significance test shows that the performance of GNNs on the original graphs is significantly different than the performance of the feature-only baseline, i.e., GNNs significantly outperform the baseline on all datasets except on WebKB where the baseline significantly outperforms the GNNs.
Mapping our results back to the cluster assumption and the uncertainty coefficient, we notice that when $U(L|C)$ is high, i.e., for CORA-ML (.691), CiteSeer (.647) and PubMed (.673), GNNs are able to consistently outperform the baseline. Meanwhile, when $U(L|C)$ is low, i.e., for WebKB (.320), GNNs are not useful for the task.% we notice that GNNs are able to consistently outperform the baseline in cases where nodes within a community are assumed to share the same label, i.e., CORA-ML, CiteSeer, PubMed and CORA-FULL, where $U(L|C)$ is $.691, .647, .673, .479$ respectively. Meanwhile, GNNs are not successful when $U(L|C)$ is low, i.e., $.32$ on WebKB.


\para{Ablation results.} On citation datasets, the accuracy drop on the SBM graphs is smaller than for the other two ablation models (CM and random graphs).
As SBM graphs preserve the community structure, this observation shows a noticeable impact of communities on node classification in citation datasets. However, this behavior is not always demonstrated on the Twitter dataset.
On contrary, on the Twitter dataset, we observe an overlap in the performances on the original graph and the ablation models. This performance overlap is even more prominent on WebKB.
The SBM graphs generally gain the lowest accuracy on the WebKB dataset, showing a negative effect of preserving communities in this dataset.
These observations can again indicate that communities are boosting the prediction for the citation datasets (where $U(L|C)$ is high) while hindering it for the WebKB dataset (where $U(L|C)$ is low).% \dhe{relate this finding to the uncertainty coefficient}

% \para{Hubs.} Comparing the performance on CM graphs to random graphs, we observe a higher accuracy on random graphs in most cases.
% % what it means
% This highlights the role of hubs which are preserved in the CM graphs and eliminated in the random graphs.
% % implication/explanation
% The existence of hubs and the absence of the original community structure in CM graphs could be causing features to spread faster across nodes with different labels comparing to the random graphs, hence causing oversmoothing.
 

\subsection{Discussion}
\label{sec:uncertainty-result}
% \hussain{change the way you tell this mini story: first we perform the perturbation, we compute U(L|C), we compute U(L|C) since it is realistic (we might need to mention this thing earlier on, maybe in the analysis section), then we evaluate GCN and show that there is a positive correlation with the estimated one. The impact is that this metric can be used even with few labeled data points and indicate whether GNNs are applicable}
% Motivation: previous results suggest ULC can be used as a guideline
%\para{Correlation with uncertainty coefficient.}
In our experiments, we observe that the uncertainty coefficient is high for the citation datasets, relatively low for Twitter, and much lower for WebKB.
This correlates with the classification performance on citation datasets that show (a) a consistent performance on the original graphs and (b) a better accuracy on SBM graphs comparing to the other ablations.
%We do not observe similar results on other two datasets and this is reflected by the uncertainty coefficient as well.
On contrary, in the Twitter dataset, where GNNs only outperform the baseline by a small margin, the behavior is reflected in the coefficient value that is smaller than in three out of four citation datasets.
For WebKB, the coefficient is particularly low following the observations that GNNs are unable to beat the simple baseline on the original network.

Our observation suggest that the uncertainty coefficient can indicate whether GNNs are applicable depending on the relationship between the communities and labels.
To shed more light on the correlation between the uncertainty coefficient and the classification performance of GNNs, we now study the change of both GNN accuracy and the measured uncertainty coefficient on the given datasets after applying additional community perturbations.
%Our evaluation results suggest that community-label correlation (measured by the empirical $U(L|C)$ metric) can act as a guideline to when GNNs are applicable.
% Goal: defend that U(L|C) could be used as a guideline
%Therefore, we aim to empirically support this finding through \textit{community perturbations} on the given datasets.
% Method: applying perturbation and measuring U(L|C) and accuracy
%\para{Method.}
Particularly, we start with the SBM networks for each dataset and we perform the following perturbations.
We randomly select a fraction of nodes and assign them to different communities by simply swapping the nodes position in the network.
Then we gradually increase the fraction of the selected nodes to obtain a spectrum of the uncertainty coefficient.
Finally, we compute $U(L|C)$ and the accuracy of the GCN model on each of the obtained graphs and show the correlation between the two measures.
We choose the SBM networks for this experiment to guarantee that the node swapping only changes nodes' communities and not their importance.
We expect that these perturbations increasingly reduce $U(L|C)$ when the cluster assumption holds.




%\para{Results.}
% Result: we show that estimated U(L|C) positively correlates with accuracy
% We empirically show that $U$ changes similar to $U$ with increasing perturbations (cf. Figure~\ref{fig:swap} [top]), which supports that $U$ can be used as an estimate of the real value $U$.\dhe{check the comment above and change accordingly.}
We show that $U(L|C)$ decreases and then converges for the first 5 datasets datasets (cf. Figure~\ref{fig:swap} [top]), supporting that the community perturbations decrease the correlation between communities and labels.
In these cases, the GNN accuracy has a positive correlation with $U(L|C)$ (cf. Figure~\ref{fig:swap} [bottom]).
However, when community perturbations do not reduce the correlation between communities and labels, $U(L|C)$ is already at a convergence level.
That is the case where GNNs were not able to outperform the feature-based baseline, i.e., WebKB.
By reading the bottom row of Figure~\ref{fig:swap}, we see that when $U(L|C)$ is below $0.3$, the accuracy becomes unacceptably low. On the contrary, if $U(L|C)$ is above $0.7$, the accuracy is high enough for the respective dataset.
% \hussain{talk about when the accuracy becomes bad and set the ground for a threshold}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{sbm-swap-ulc.eps}
    \includegraphics[width=\linewidth]{sbm-swap-correlation-known.eps}
    \caption{The figure in the top row shows the calculated $U(L|C)$ for each dataset. The swap fraction represents the fraction of nodes which changed their community. We see a decline in the coefficient with increasing swapping fraction, and then a convergence. This line is already converging in WebKB as the measure is already low in the original network. The figure in the bottom shows the test accuracy with changing $U(L|C)$. We see a positive correlation between the uncertainty coefficient and the accuracy, which is weak for Twitter, and non-existent for WebKB supporting our observations from above.}
    \label{fig:swap}
\end{figure}


\para{Guideline for application of GNNs.} %\tdu{Guideline or similar instead of Recommendation?}
To verify whether a GNN model is applicable on a certain real-world dataset, we suggest the following two-step guideline based on the previous observations.
\begin{itemize}
    \item The first step is to perform community detection on the dataset, and inspect the uncertainty coefficient for it.
If the coefficient is particularly low, e.g., below $0.3$, there is a high confidence that GNNs will not work.
If the coefficient is particularly high, e.g., above $0.7$, it is likely that GNNs can exploit the network structure and be helpful for the prediction task.
Otherwise, if the value is inconclusive, e.g., around $0.5$, we advise to perform the second step.
    \item The second step involves gradual community perturbations and inspection of the respective uncertainty coefficient.
If the value of the coefficient decreases with more perturbations, this supports that the cluster assumption holds in the original graph, and GNNs are applicable.
Otherwise, if it does not decrease, the cluster assumption most likely does not hold in the first place, and feature-based methods are more advisable than GNNs.
\end{itemize}

% The smaller the coefficient is, the less likely the GNNs are to be useful.
% Then one should perform the increasing community perturbation explained above and measure $U(L|C)$ respectively. If $U(L|C)$ declines with increasing perturbations, it means that the GNNs can improve over feature-only methods. If $U(L|C)$ does not decline, using GNNs could hinder the classification accuracy, and it is advisable to use a feature-only approach. \hussain{Is it better now?} \dhe{maybe we can explain guidelines in two steps: the first step is the inspection of the uncertainty coefficient. if it is lower than some value than it is a strong indication that the GNNs are not applicable. in particular if it is lower than e.g. 0.1 then most probably the GNNs will not work. opposite for high values, e.g. 0.8 or higher. these thresholds we should be able to read from the figure 2, right? the second step is optional, i.e. in the cases where the uncertainty coefficient is inconclusive, e.g. maybe .5 then perturbation experiment can be performed.} \hussain{How can we tell what the thresholds are? We don't have enough evidence. Or should we just use terms like `high' or `low'?} \dhe{we can deduce the thresholds from our perturbation experiments, right? just check the bottom row of Figure 2 and decide what is acceptable accuracy and then read off the corresponding uncertainty coefficient.}

% \para{Summary.}
% Mapping our results back to the assumptions we have mentioned about the given datasets (in Section~\ref{sec:dataset-interest}), we notice that GNNs were able to consistently outperform the baseline only in cases where nodes within a community are assumed to share the same label, i.e., citation datasets.
% We also see that for these datasets, preserving communities resulted in the best accuracy compared to the other ablation models.
% On the contrary, the baseline was not outperformed consistently for the other two datasets, and SBM graphs did not preserve the most accuracy among the other ablation models.
